Toward Annotator Group Bias in Crowdsourcing

Crowdsourcing has emerged as a popular approach for collecting annotated data to train supervised machine learning models. However, annotator bias can lead to defective annotations. Though there are a few works investigating individual annotator bias, the group effects in annotators are largely overlooked. In this work, we reveal that annotators within the same demographic group tend to show consistent group bias in annotation tasks and thus we conduct an initial study on annotator group bias. We first empirically verify the existence of annotator group bias in various real-world crowdsourcing datasets. Then, we develop a novel probabilistic graphical framework GroupAnno to capture annotator group bias with a new extended Expectation Maximization (EM) training algorithm. We conduct experiments on both synthetic and real-world datasets. Experimental results demonstrate the effectiveness of our model in modeling annotator group bias in label aggregation and model learning over competitive baselines.

==> related_literature.tex <==
% % . By using optimized weights for answers derived from participants’ confidence, we are able to build a super player





% % It is therefore of societal and ethical importance to ask whether these algorithms can be discriminative on grounds such as gender, ethnicity, or health status

% % Sometimes it may be inherent to the data sources used; but even when the sensitive attributes have been suppressed from the input, a well trained machine learning algorithm may still discriminate on the basis of such sensitive attributes because of correlations existing in the data.

% % call for the development of data mining systems which are discrimination-conscious by-design.

% % Three approaches are conceivable for discrimination prevention: preprocessing by means of transforming the source data; inprocessing by means of integrating the anti-discrimination constrains in the design of algorithm; postprocessing by means of modifying the results of data mining models
% % Pre-processing approaches including correcting the training data; inprocessing approaches including na¨ıve bayes models, logistic regression, decision trees, hinge loss, support vector machines, adaptive boosting and classification; post-processing approaches including classification, rule and pattern mining; simultaneous discrimination prevention and privacy protection considering k-anonymity, t-closeness and differential privacy models [3, 8, 11, 7, 6, 10, 9].
% % [Algorithmic Bias: From Discrimination Discovery to Fairness-aware Data Mining]



% % One important problem is to identify the true information (i.e., the truths) among conflicting sources of data. It is intuitive to trust reliable sources more when deriving the truths, but it is usually unknown which one is more reliable a priori
% % They used difference loss functions and used an optimization framework to minimize the reliability distance between the truth and descriptions obtained from multiple sources 
% % [Resolving Conflicts in Heterogeneous Data by Truth Discovery and Source Reliability Estimation]



% % it is important to take fairness issues into consideration while designing and engineering these types of systems. Such systems can be used in many sensitive environments to make important and life-changing decisions; thus, it is crucial to ensure that the decisions do not reflect discriminatory behavior toward certain groups or populations



% % discrimination prevention by means of fairness-aware data mining, developing data mining systems which are discrimination-conscious by-design
% % [A methodology for direct and indirect discrimination prevention in data mining. 







% % Our findings suggest that annotator bias should be monitored during dataset creation, and that test set annotators should be disjoint from training set annotators
% % [Are We Modeling the Task or the Annotator? An Investigation of Annotator Bias in Natural Language Understanding Datasets]



% % We used Amazon Mechanical Turk (AMT) as our primary source of annotations. Overall, a total of over 33, 000 unique workers contributed to the dataset.
% % Large number of workers through platforms such as Amazon Mechanical Turk
% % Connecting Language description and Vision - crowdsourcing technique is being used
% % [Visual Genome: Connecting Language and Vision Using Crowdsourced Dense Image Annotations]



% % The analysis of crowdsourced annotations in natural language processing is concerned with identifying (1) gold standard labels, (2) annotator accuracies and biases, and (3) item difficulties and error patterns. Traditionally, majority voting was used for 1, and coefficients of agreement for 2 and 3. 
% % Lately, model-based analysis of corpus annotations have proven better at all three tasks.

% % [Comparing Bayesian Models of Annotation]


% % No matter how precise a language user might be, language interpretation is subjective.
% % Outcomes: (a) Come up with a method to quantify reliability between annotations provided by multiple annotators in conference annotation, (b) distance measure to capture partial disagreement between annotators
% % “Lack of consistency is a problem - prior literature studies reliability between data annotators”
% % [Computing Reliability for Coreference Annotation]



% % Various measures are used to estimate reliability of manually annotated data such as (Cohen’s κ, Scott’s π, binary and weighted Krippendorff ’ s α
% % Experimentally showed that weighted α is the most reliable metrics
% % [Weighted Krippendorff’s alpha is a more reliable metrics for multi- coders ordinal annotations: experimental studies on emotion, opinion and coreference annotation] 



% % One of the biggest challenges of crowdsourcing is aggregating the answers collected from the crowd since the workers might have wide-ranging levels of expertise. In order to tackle this challenge, many aggregation techniques have been proposed.

% % One of the most important technical challenges of crowdsourcing is answer aggregation [17], which aggregates a set of human answers into a single value. In our setting, we consider a broad class of problems in which there is an objective ground truth external to human judgment; i.e. each question has an exact answer but no one knows what it is. The goal of answer aggregation is to find this hidden ground truth from a set of answers given by the crowd workers. “This goal is, however, difficult to achieve for various reasons - expertise, bias…”
% % main reasons.

% % Non-iterative: uses heuristics to compute a single aggregated value of each question separately. One simple approach is Majority Decision (MD)
% % Iterative: performs a series of iterations, each consisting of two updating steps: (i) updates the aggregated value of each question based on the expertise of workers who answer that question, and (ii) adjusts the expertise of each worker based on the answers given by him

% % understanding the performance implications of these techniques is challenging, since each of them has distinct characteristics. One, for example, may achieve very high accuracy over certain types of workers, while another is sensitive to spammers.

% % “Effect on performance due to bias is not well understood.”

% % [An Evaluation of Aggregation Techniques in Crowdsourcing]



% % Several approaches for debiasing gender bias - retraining and inference are two broad ways of achieving it. Retraining methods tend to address gender bias in its early stages or even at its source. However, retraining a model on a new data set can be costly in terms of resources and time. Inference
% % methods, on the other hand, do not require models to be retrained; instead, they patch existing models to adjust their outputs providing a testing-time debiasing

% % [Mitigating Gender Bias in Natural Language Processing: Literature Review]




% % Gender bias is the preference or prejudice toward one gender over the other (Moss-Racusin et al., 2012).
% % [Science Faculty’s Subtle Gender Biases Favor Male Students]


% % Gender bias exist in pre-trained models {reference below}, training data, and algorithm
% % [Learning Gender-Neutral Word Embeddings]
% % [Word Embeddings Quantify 100 Years of Gender and Ethnic Stereotypes]

% % Even amplify biases present in the training sets (Zhao et al., 2017).
% % [Men Also Like Shopping: Reducing Gender Bias Amplification Using Corpus-Level Constraints.]


% % Fairness studies are important because…
% % Machine learning is no longer just the engine behind ad placements and spam filters: it is now used to filter loan applicants, deploy police officers, and inform bail and parole decisions, amongst other things.

% % Causes of unfairness (a) But if we train a group-blind classifier to minimize overall error, if it cannot simultaneously fit both populations optimally, it will fit the majority population. This leads to a different (and higher) distribution of errors in the minority population; (b) bias encoded from data source

% % [The Frontiers of Fairness in Machine Learning]

% % Types of bias:
% % (a) Label bias emerges when the distribution of the dependent variable in the data source diverges substantially from the ideal distribution [Predictive Biases in Natural Language Processing Models: A Conceptual Framework and Overview]
% % (b) Bias due to provided contextual information: for subjective tasks such as sentiment analysis, sarcasm detection providing too little or too much context would bias the label created by the annotators. we show that providing too little context can result in noisy and uncertain annotations, whereas providing too strong a context may cause it to outweigh other signals [ConStance: Modeling Annotation Contexts to Improve Stance Classification]
% % (c) Selection Bias : Selection bias emerges due to non-representative observations. I.e., when the users generating the training (source) observations differ from the user distribution of the target, where the model will be applied [Predictive Biases in Natural Language Processing Models: A Conceptual Framework and Overview]



% % Our findings show that the proposed approach successfully identifies bias and that demographic features, such as first language, age, and education, correlate with significant performance differences.

% % [Identifying and Measuring Annotator Bias Based on Annotators’ Demographic Characteristics]


% % [Data statements for natural language processing: Toward
% % mitigating system bias and enabling better science.]

% % [Are We Modeling the Task or the Annotator? An Investigation of Annotator Bias in Natural Language Understanding Datasets]


% Fairness issues are being increasingly studied as machine learning systems are being increasingly used in sensitive applications such as informing bail and parole decisions, deploy troops, filter loan applications [The Frontiers of Fairness in Machine Learning]. Biases refer to cases where computer systems “systematically and unfairly discriminate against certain individuals or groups of individuals in favor of others” [Bias in Computer Systems]. For example gender bias is preference or prejudice towards one gender over another [Science Faculty’s Subtle Gender Biases Favor Male Students].

% Bias is caused due to pre-existing societal norms, data source, data labeling, training algorithms, and post-processing models. NLP system typically involve algorithms trained on particular datasets [Data statements for natural language processing: Toward mitigating system bias and enabling better science.]. Data source bias or selection bias emerges when the source distribution differ from the target distribution where the model will be applied.  Data labeling bias is when the distribution of the dependent variable in the data source diverges from the ideal distribution that leads to label bias [Predictive Biases in Natural Language Processing Models: A Conceptual Framework and Overview]. This is caused by differences in data annotators and is amplified based by task difficulty, task ambiguity, and the amount of contextual information made available to the data annotators [ConStance: Modeling Annotation Contexts to Improve Stance Classification]. In this work we focus on bias created by data annotators. 

% and  data labels An example 

% NLP systems are algorithms, trained on specific datasets, that does some kind of natural language processing 


%  Types: (a) show that in some cases, system bias reflects biases in society; these are pre-existing biases with roots in social institutions, practices and attitudes, (b) (e.g., the order in which an algorithm processes data) can result in bias when used in real world contexts; these technical biases, and (c) A third source of bias, emergent bias, occurs when a system designed for one context is applied in another (e.g., with a different population). [Bias in Computer Systems]. Such biases have several detrimental effects on the NLP systems such as discriminating certain groups of people in sensitive applications [A methodology for direct and indirect discrimination prevention in data mining.]. 

% Annotator bias due to demographic can arise due to gender [Do women perceive hate differently:
% Examining the relationship between hate speech, gender, and agreement judgments], racial [Racial bias in hate speech and abusive language detection datasets], expertise [Are we modeling the task or the annotator? an investigation of annotator bias in natural language understanding datasets], political [Impact of Politically Biased Data on Hate Speech Classification]


% Another approach is to mitigate the bias. Several approaches have been proposed for bias mitigation. Using data statements or standardized information to mitigate system bias in NLP technology [Data statements for natural language processing: Toward mitigating system bias and enabling better science.], using disjoint annotators in the training and testing sets [Are We Modeling the Task or the Annotator? An Investigation of Annotator Bias in Natural Language Understanding Datasets], developing data mining systems which are discrimination conscious by design [A methodology for direct and indirect discrimination prevention in data mining.], retraining methods, patching existing models by adjusting their outputs Mitigating Gender Bias in Natural Language Processing: Literature Review]

% Very little prior work has been done on fairness for text classification task. Most of the existing work discusses the implications of fairness, but do not provide strategies to mitigate them [The Social Impact of Natural Language] [Racial Disparity in Natural Language Processing: A Case Study of Social Media African-American English.

% An aspect that is sparsely investigated in this context is the relation between annotators’ demographic features and a potential bias in the data set. Previous work has done exploratory studies on how demographic features such as age, gender, education, and first language impact annotation of hateful content. [Identifying and Measuring Annotator Bias Based on Annotators’ Demographic Characteristics]. However, how to mitigate the potential bias created by demographic features is not studied.

% Our work adds to this growing body of machine learning fairness research with a novel approach to


